The failure of cut-elimination in cyclic proof for first-order logic with inductive definitions

A cyclic proof system is a proof system whose proof figure is a tree with cycles. The cut-elimination in a proof system is fundamental. It is conjectured that the cut-elimination in the cyclic proof system for first-order logic with inductive definitions does not hold. This paper shows that the conjecture is correct by giving a sequent not provable without the cut rule but provable in the cyclic proof system.

==> author.tex <==
\author[1,$\ast$]{Yukihiro Masuoka}
\author[1]{Makoto Tatsuta}

\address[1]{\orgdiv{Department of Informatics}, \orgname{The Graduate University for Advanced Studies}, \orgaddress{\street{Chiyoda-ku}, \postcode{101-8430}, \state{Tokyo}, \country{Japan}}}

\corresp[$\ast$]{Corresponding author. \href{email:yukihiro\_m@nii.ac.jp}{yukihiro\_m@nii.ac.jp}}

==> oupsettings.tex <==
%\journaltitle{Journal of Logic and Computation}
\journaltitle{}
\DOI{ }
\copyrightyear{2021}
\pubyear{ }
\access{ }
\appnotes{ }

\firstpage{1}
